Modeling and Control of Sustainable Transitions through Opinion-Behavior Coupling in Heterogeneous Networks

Understanding how sustainable behaviors spread within heterogeneous societies requires the integration of behavioral data, social influence mechanisms, and structured approaches to control. In this paper, we propose a data-driven computational framework for coupled opinion-adoption dynamics in social systems. Each node in the multilayer network represents a community characterized by a specific age group and mobility level, derived from large-scale survey data on the predisposition to adopt electric vehicles in Northern Europe. The proposed model captures three mechanisms: behavioral contagion through social and informational diffusion, abandonment driven by dissatisfaction, and feedback between opinions and adoption levels through social influence. Analyzing the equilibrium points of the coupled system allows us to derive the conditions that enable large-scale adoption. We empirically calibrate the model using data to construct synthetic populations and social similarity networks, which we use to explore targeted interventions that promote sustainable transitions. Specifically, the analysis focuses on two types of control strategies: opinion-based policies, which act on the social network layer, and policies that aim to improve experience and reduce dissatisfaction. Simulation results show that the latter ensure more stable and long-term adoption, offering concrete insights for designing effective interventions in sociotechnical transitions toward sustainability.

==> Plots/README <==
Bachelor and Master thesis template based on
TOPtesi bundle version 6.x
(TOPtesi Copyright 2008-2018 Claudio Beccari
LaTeX Project Public Licence LPPL v.1.3c (or later))

For details and manuals on the TOPtesi package plese
make reference to the online documentation.

The frontispiece is compatible with that available on
the Politecnico Student Guide 2017-2018.

To modify the frontispiece, open title.tex 
Comment/uncomment your degree programm (lines 7-8 and 
10-11).
Write your thesis title (on line 12).
Insert your name and the name of your supervisor(s)
(within the minipage block).
Write the academic year (at the end of the center
block).

Save the changes.
Open toptesi_template.tex and compile it.


The set up is suitable to write the thesis both
in Italian and English. 
For the English version, just uncomment line 56
(\english command after \begin{document}).
No other action are required.

references.bib contains the references you need.

Pictures is the images folder.

Part_II contains the .tex file of the second part of
the thesis (just to show how to include different
.tex files).
